Light Affine Logic (Proof Nets, Programming Notation, P-Time Correctness and Completeness)

This paper is a structured introduction to Light Affine Logic, and to its intuitionistic fragment. Light Affine Logic has a polynomially costing cut elimination (P-Time correctness), and encodes all P-Time Turing machines (P-Time completeness). P-Time correctness is proved by introducing the Proof nets for Intuitionistic Light Affine Logic. P-Time completeness is demonstrated in full details thanks to a very compact program notation. On one side, the proof of P-Time correctness describes how the complexity of cut elimination is controlled, thanks to a suitable cut elimination strategy that exploits structural properties of the Proof nets. This allows to have a good catch on the meaning of the ``paragraph'' modality, which is a peculiarity of light logics. On the other side, the proof of P-Time completeness, together with a lot of programming examples, gives a flavor of the non trivial task of programming with resource limitations, using Intuitionistic Light Affine Logic derivations as programs.

==> expressiveness.tex <==
%auto-ignore
\section{The expressive power of ILAL}
All polytime functions can be expressed inside ILAL. This can be
proved by a more or less straightforward 
rephrasing of Girard's proof, namely by
encoding polytime Turing machines. For lack of space, we
cannot afford the full proof: we shall just give a few
hints about the encoding of data types in our system (up
to the only interesting case: the predecessor function) leaving
the rest to the reader.

Since our syntax is not particularly friendly, we introduce
the following convention:

\[(M\;N) = x[^{(z\;N)}/_x][^M/_z] \]
where $x$ and $z$ are fresh variables of the suitable types.



==> integers.tex <==
%auto-ignore
\subsection{Integers}
\label{subsection:integers}
The type {\bf int} of {\em tally} integers is:
\[ \forall \alpha. !(\alpha \linear \alpha) \linear \S(\alpha \linear \alpha)\]
The tally integer $n$ is:\vspace*{0.1cm}\\
$n = \Lambda \alpha.\lambda x:!(\alpha \linear \alpha).$\vspace*{0.1cm}\\
$\hspace*{1cm}\S(\lambda y:\alpha. 
(w_1\dots(w_n\;y)\dots))[^x\!/_{w_1},\dots,^x\!/_{w_n}]$\vspace*{0.2cm}\\
The first interesting term is the successor function
\mbox{$succ: {\bf int} \linear {\bf int}$}. 
The usual $\lambda$-calculus definition of $succ$ is 
\[\lambda n.\lambda x. \lambda y.(x\;(n\;x\;y))\]
However, there is {\em no way} to put boxes around this term
in such a way as to obtain a correct term of ILAL of the required type. 
The problem is that
$n$ must have type ${\bf int}$ (so, it cannot appear inside a box), 
while the sub-term $\lambda y.(x\;(n\;x\;y))$ must have type $\S(\alpha \linear
\alpha)$, so it must be inside a $\S$-box. 
This is the main reason why we {\em need} explicit
substitutions in the calculus.

Then, we may define $succ: {\bf int} \linear {\bf int}$ as follows:\vspace*{.2cm}\\
$succ = \lambda n:{\bf int}.\Lambda \alpha.
\lambda x:!(\alpha \linear \alpha).$\vspace*{.1cm}\\
$\hspace*{1cm}\S(\lambda y:\alpha.(w_1(w_2\;y)))[^x/_{w_1},^{((n \alpha)\;x)}/_{w_2}]$\vspace*{.2cm}\\
where $w_1$ and $w_2$ have the same type of $x$ and $((n \alpha)\;x)$, 
namely $\S(\alpha \linear \alpha)$.

As an example, in Figure 4 we trace 
the reduction of $(succ\;1)$.

Similarly, addition is the term 
$+: {\bf int}\linear {\bf int} \linear {\bf int}$
defined as follows\vspace*{.2cm}:\\
$+ = \lambda n_1:{\bf int}.\lambda n_2:{\bf int}.\Lambda \alpha.\lambda x:!(\alpha \linear \alpha).$\vspace*{.1cm}\\
$\hspace*{1cm}\S(\lambda y:\alpha.(w_1(w_2\;y)))[^{((n_1 \alpha)\;x)}/_{w_1},^{((n_2 \alpha)\;x)}/_{w_2}]$\vspace*{.2cm}\\
%where $w_1$ and $w_2$ have type $\S(\alpha \linear \alpha)$.\\
Multiplication $\times : !{\bf int} \linear {\bf int} 
\linear \S({\bf int})$ is defined by iteration of $+$\vspace*{.2cm}:\\
$\times = \lambda n:!{\bf int}.\lambda m:{\bf int}.\Lambda \alpha.$\vspace*{.1cm}\\
$\hspace*{1cm}\S(w\;0)[^{((m\;{\bf int})\;!(\lambda y:{\bf int}.(+\;n\;y)))}/_w]$\vspace*{.2cm}\\
where $w:\S({\bf int} \linear {\bf int})$.

In general, we have the following\vspace{.3cm}\\
{\bf Iteration Principle} Let $x:B \vdash M: A\linear A$ and 
$\Delta \vdash N:A$. Then
\[y:!B,\S(\Delta),m:{\bf int} \vdash \S(w\;N)[^{(m\;A\;!(M)[^y/_x])}/_w]: \S(A)\]
%where $w:\S(A\linear A)$.\\
Note in particular that 
\[succ_k = \lambda n:!^k{\bf int}.!^k(succ\;n):!^k{\bf int} 
\linear !^k{\bf int}\]
and 
\[0_k = !^k(0):!^k{\bf int}\]
By applying iteration, we
get the term $coer_k :$ \mbox{${\bf int}\linear \S!^k{\bf int}$} defined as follows:
\[coer_k = \lambda m:{\bf int}.\S(w\;0_k)[^{(m\;!^k{\bf int}\;!(succ_k))}/_w]\]
Note that $coer_k$ is essentially the identity on integers, 
but it changes the type, and according to Girard we call it
a {\em coercion}.

In a similar way we may define coercions of type 
${\bf int}\linear \S^p!^k{\bf int}$ for any $p>0$. Note now that
\[x:\S!{\bf int}, y:\S{\bf int} \vdash \S(\times\;x\;y):\S^2{\bf int}\]
By composing with the coercions ${\bf int}\linear \S!{\bf int}$
and ${\bf int}\linear \S{\bf int}$ we get a new definition of 
multiplication $\times'$ of type ${\bf int}\linear{\bf int}\linear
\S^2{\bf int}$.

More generally, following Girard, it is easy
to prove that any polynomial of degree $n$ can be represented in the system by
a term of type ${\bf int}\linear \dots {\bf int}\linear \S^p{\bf int}$

